Adversarial Representation Learning With Closed-Form Solvers

Adversarial representation learning aims to learn data representations for a target task while removing unwanted sensitive information at the same time. Existing methods learn model parameters iteratively through stochastic gradient descent-ascent, which is often unstable and unreliable in practice. To overcome this challenge, we adopt closed-form solvers for the adversary and target task. We model them as kernel ridge regressors and analytically determine an upper-bound on the optimal dimensionality of representation. Our solution, dubbed OptNet-ARL, reduces to a stable one one-shot optimization problem that can be solved reliably and efficiently. OptNet-ARL can be easily generalized to the case of multiple target tasks and sensitive attributes. Numerical experiments, on both small and large scale datasets, show that, from an optimization perspective, OptNet-ARL is stable and exhibits three to five times faster convergence. Performance wise, when the target and sensitive attributes are dependent, OptNet-ARL learns representations that offer a better trade-off front between (a) utility and bias for fair classification and (b) utility and privacy by mitigating leakage of private information than existing solutions.

==> conclusion.tex <==
\section{Concluding Remarks}

Adversarial representation learning is a minimax theoretic game formulation that affords explicit control over unwanted information in learned data representations. Optimization algorithms for ARL such as stochastic gradient descent-ascent (SGDA) and their variants are sub-optimal, unstable and unreliable in practice. In this paper, we introduced OptNet-ARL to address this challenge by employing differentiable closed-form solvers, such as kernelized ridge regressors, to model the ARL players that are downstream from the representation. OptNet-ARL reduces iterative SGDA to a simple optimization, leading to a fast, stable and reliable algorithm that out-performs existing ARL approaches on both small and large scale datasets. 

\vspace{5pt}
\noindent\textbf{Acknowledgements:} This work was performed under the following financial assistance award 60NANB18D210 from U.S. Department of Commerce, National Institute of Standards and Technology.

==> related-work.tex <==

\section{Prior Work}

\noindent\textbf{Adversarial Representation Learning:} The basic idea of learning data representations with controllable semantic information has been effective across multiple topics. Domain adaptation~\cite{ganin2015unsupervised, ganin2016domain, tzeng2017adversarial}, where the goal is to learn representations that are invariant to the domain, is one of the earliest applications of ARL. More recently, adversarial learning has been extensively used \cite{edwards2015censoring,beutel2017data,xie2017controllable,zhang2018mitigating,song2018learning,elazar2018adversarial,bertran2019adversarially,roy2019mitigating,creager2019flexibly} and advocated \cite{madras2018learning} for the task of learning fair, invariant or privacy preserving representations of data. All of the aforementioned approaches represent each entity in ARL by neural networks and optimize their parameters through stochastic gradient descent-ascent (SGDA). As we show in this paper, SGDA is unstable and sub-optimal for learning. Therefore, we trade-off model expressively for ease of learning through a hybrid approach of modeling the encoder by a deep neural network and target and adversary with closed-form regressors. Such a solution reduces alternating optimization into a simple optimization problem which is much more stable, reliable and effective. Table~\ref{tbl-comparison} shows a comparative summary of ARL approaches.

\noindent\textbf{Optimization in Minmax Games:} A growing class of learning algorithms, including ARL, GANs etc., involve more than one objective and are trained via games played by cooperating or dueling neural networks. An overview of the challenges presented by such algorithms and a plausible solution in general $n$-player games can be found in \cite{letcher2019differentiable}. In the context of two-player minimax games such as GANs, a number of solutions~\cite{mescheder2017numerics,nagarajan2017gradient,balduzzi2018mechanics,daskalakis2018limit,jin2019local,gidel2018variational} have been proposed to improve the optimization dynamics, many of them relying on the idea of taking an extrapolation step \cite{korpelevich1976extragradient}. 
For example,~\cite{mescheder2017numerics} deploys some regularizations to encourage  agreement between different players and improve the convergence properties.
In another example,~\cite{nagarajan2017gradient} uses double gradient to stabilize the optimization procedure. 
In contrast to all of these approaches, that work with the given fixed models for each player, we seek to change the model of the  players in the ARL setup for ease of optimization. In the context of ARL, \cite{sadeghi2019global} considers the setting where all the players, including the encoder, are linear regressors. While they obtained a globally optimum solution, the limited model capacity hinders the flexibility (cannot directly use raw data), scalability and performance (limited by pre-trained features) of their solution. In this paper we advocate the use of ridge regressors (linear or kernel) for the target and adversary, while modeling the encoder as a deep neural network. This leads to a problem that obviates the need for gradient descent-ascent and can instead be easily optimized with standard SGD. Not only does this approach lead to stable optimization, it also scales to larger datasets and exhibits better empirical performance.

\begin{table}[t]
\centering
\caption{Comparison between different ARL methods ($n$: sample size, $b$: batch size).}
\resizebox{\textwidth}{!}{
\begin{tabular}{ p{3.0cm} p{4.9cm} p{2.25cm} p{1.4cm} p{1.95cm} p{1.7cm}}
\toprule
\textbf{\hfil Method} &\textbf{Encoder / Target \& Adversary}& \hfil \textbf{Optimization}& \textbf{Scalability}   & \textbf{\hfil Enc Soln}& \textbf{Input Data}\\
\midrule
 \hfil \textbf{SGDA-ARL}~\cite{xie2017controllable,madras2018learning} & \hfil deep NN / shallow NN &  alternating SGD &  \hfil $\geq \mathcal{O}(b^3)$& \hfil unknown & \hfil raw data\\ 
 \textbf{Kernel-SARL}~\cite{sadeghi2019global} & \hfil kernel regressor / linear & \hfil closed-form&  \hfil $\mathcal{O}(n^3)$ & \hfil global optima & \hfil features\\  
 \midrule
 \textbf{\hfil OptNet-ARL} (ours) &  \hfil deep NN / kernel regressor  & \hfil SGD & \hfil $\mathcal{O}(b^3)$ & \hfil local optima & \hfil raw data\\
 \toprule
\end{tabular}\label{tbl-comparison}
}
\end{table}

\noindent\textbf{Differentiable Solvers:} A number of recent approaches have integrated differentiable solvers, both iterative as well as closed-form, within  end-to-end learning systems. Structured layers for segmentation and higher order pooling were introduced by \cite{ionescu2015training}. Similarly \cite{valmadre2017end} proposed an asymmetric architecture which incorporates a Correlation Filter as a differentiable layer. Differential optimization as a layer in neural networks was introduced by \cite{amos2017optnet,agrawal2019differentiable}. More recently, differentiable solvers have also been adopted for meta-learning \cite{bertinetto2018meta,lee2019meta} as well. The primary motivation for all the aforementioned approaches is to endow deep neural networks with differential optimization and ultimately achieve faster convergence of the end-to-end system. In contrast, our inspiration for using differential closed-form solvers is to control the non-convexity of the optimization in ARL, in terms of stability, reliability and effectiveness.
